LLM Unlearning via Loss Adjustment with Only Forget Data

Unlearning in Large Language Models (LLMs) is essential for ensuring ethical and responsible AI use, especially in addressing privacy leak, bias, safety, and evolving regulations. Existing approaches to LLM unlearning often rely on retain data or a reference LLM, yet they struggle to adequately balance unlearning performance with overall model utility. This challenge arises because leveraging explicit retain data or implicit knowledge of retain data from a reference LLM to fine-tune the model tends to blur the boundaries between the forgotten and retain data, as different queries often elicit similar responses. In this work, we propose eliminating the need to retain data or the reference LLM for response calibration in LLM unlearning. Recognizing that directly applying gradient ascent on the forget data often leads to optimization instability and poor performance, our method guides the LLM on what not to respond to, and importantly, how to respond, based on the forget data. Hence, we introduce Forget data only Loss AjustmenT (FLAT), a "flat" loss adjustment approach which addresses these issues by maximizing f-divergence between the available template answer and the forget answer only w.r.t. the forget data. The variational form of the defined f-divergence theoretically provides a way of loss adjustment by assigning different importance weights for the learning w.r.t. template responses and the forgetting of responses subject to unlearning. Empirical results demonstrate that our approach not only achieves superior unlearning performance compared to existing methods but also minimizes the impact on the model's retained capabilities, ensuring high utility across diverse tasks, including copyrighted content unlearning on Harry Potter dataset and MUSE Benchmark, and entity unlearning on the TOFU dataset.

==> LLM_Unlearning_arxiv/src/01-intro.tex <==
\section{Introduction}
\label{sec:intro}

The widespread integration of Large Language Models (LLMs) into daily applications has raised significant concerns regarding the trustworthiness of such models. Their outputs may contain sensitive, private, or illegal content~\cite{karamolegkou2023copyright,patil2023can}, reflect societal biases~\cite{motoki2024more,yu2023unlearning}, or provide harmful instructions~\cite{yao2023large,li2024wmdp,barrett2023identifying}. In particular, for privacy concerns, regulations~\cite{hoofnagle2019european} have been introduced, requiring applications to support the deletion of information contained in training samples upon user request. This has motivated research into machine unlearning (MU)~\cite{cao2015towards,liu2024model,fan2023salun,di2024label,liu2024rethinking}, a critical process aimed at removing the influence of specific data points, data classes, or even higher-level data concepts from trained models.



LLM unlearning~\cite{eldan2023s,yao2023large,liu2024rethinking} is part of a broader set of MU techniques aiming to make the unlearned model forget the knowledge specified in forget dataset, while preserving the model ability to accomplish tasks irrelevant to the unlearning target~\cite{liu2024rethinking,ji2024reversing}. To achieve this, existing work can be categorized into three main streams of LLM unlearning approaches: input-based, data-based, and model-based methods. Input-based methods~\cite{liu2024large,pawelczyk2023context} design input instructions to guide the original LLM towards the unlearning objective without altering the model's parameters. Data-based methods~\cite{choi2024snap} typically fine-tune models on pre-constructed desirable responses, using prompts from the forget data distribution. Model-based methods~\cite{yao2023large,chen2023unlearn} focus on modifying the weights or architecture to achieve the unlearning objective. Among these approaches, the most relevant to our work is fine-tuning the target LLM using a modified loss function, which typically incorporates two key objectives: maximizing the loss on the forget samples and minimizing (or maintaining) the loss on the retain samples.

 
\input{tables/baseline_comparison}

However, as summarized in Table~\ref{tab:baselines}, current loss adjustment-based methods either rely on retain data~\cite{maini2024tofu, liu2022continual,yao2023large}, which might not be readily available in real-world scenarios~\cite{li2024wmdp}, or utilize a reference model~\cite{rafailov2024direct,zhang2024negative,yao2023large,maini2024tofu} to maintain performance on the retain dataset, incurring additional cost during training—especially when fine-tuning a large-scale LLM. Moreover, leveraging explicit retain data or implicit knowledge from a reference LLM during fine-tuning may blur the distinction between the forget and retain data, which can lead to a trade-off between model utility and forget quality. Furthermore, fine-tuning using both retain data and forget data would require a careful design of a data mixing strategy. To preserve model utility while improving forget quality, we propose \textbf{F}orget data only \textbf{L}oss \textbf{A}justmen\textbf{T} (\textbf{FLAT}), a "flat" loss adjustment approach which adjusts the loss function using only the forget data.

Given the forget data, \method guides the LLM not only in what to forget but also in how to respond, by optimizing the $f$-divergence between the template and forget answers with respect to the forget data. The variational form of the $f$-divergence enables loss adjustment by assigning optimal importance weights to learning from template responses while forgetting the responses subject to unlearning.

Our main contributions are highlighted below:
\squishlist
    \item We identify the potential drawback of relying on retain data or a reference LLM to guide LLM unlearning. To address this, we propose \textbf{FLAT}, which facilitates LLM unlearning without requiring retain data or a reference LLM for response calibration.
    \item \method optimizes the $f$-divergence between template and forget responses to guide the LLM through the unlearning process. The variational form of $f$-divergence optimization provides a clear illustration of how to optimally balance forget quality and model utility, with theoretical guarantees.
    % \wjh{unify the saying of forget/unlearned data or answers in the paper, also for the saying of reference LLM}
    \item Extensive experiments on three unlearning tasks, including copyrighted content unlearning on the Harry Potter dataset and MUSE benchmark, as well as entity unlearning on the TOFU dataset, demonstrate the superior performance of our method, achieving both high unlearning efficiency and strong overall model utility.
    % \wjh{be more specific about tasks and datasetsd that we used,} \wyx{Done!}
\squishend


==> LLM_Unlearning_arxiv/src/02-related_work.tex <==
\section{Related Work}
\label{related_work}
\subsection{LLM Unlearning}
LLM unlearning approaches can be broadly categorized into three families: model-based methods, input-based methods, and data-based methods~\cite{liu2024rethinking}.

\paragraph{Model-based Methods}
Model-based approaches involve modifying the weights and/or architecture to achieve unlearning. These include gradient ascent (GA) and its variants~\cite{yao2023large,maini2024tofu,chen2023unlearn}, as well as model editing techniques~\cite{wu2023depn,ilharco2022editing,belrose2024leace}. The dominant approach among existing LLM unlearning methods is fine-tuning the original model based on a carefully designed unlearning objective function~\cite{chen2023unlearn,yao2023large,jia2024soul,li2024wmdp,yao2024machine,zhang2024negative}. A common strategy combines forgetting and retaining objectives, applying gradient ascent updates to undesirable data while using regular gradient descent on desirable data~\cite{chen2023unlearn,li2024wmdp}. The goal of GA is to maximize the loss on the forget data, essentially reversing the effect of gradient descent during training. Some methods employ custom loss functions that go beyond standard forgetting and retaining losses. For example, \cite{yao2023large} introduce a loss function with three components, where the custom loss reflects advanced techniques or regularization applied to the objectives. Other methods, such as DPO~\cite{rafailov2024direct}, KTO~\cite{ethayarajh2024kto}, and NPO~\cite{zhang2024negative}, utilize reference models to guide the unlearning process. 

\cite{chen2023unlearn} fine-tune an adapter over the unlearning objective, which acts as an unlearning layer within the LLM. Several works also employ assistant or reinforced LLMs to facilitate unlearning~\cite{ilharco2022editing,eldan2023s,huang2024offset}. For instance, \cite{ji2024reversing} introduce an assistant LLM that pursues the opposite of the unlearning goals—i.e., remembering forgotten documents and forgetting retained knowledge. The unlearned LLM is then derived by computing the logit difference between the original and assistant LLMs.

\paragraph{Data-based Methods}
Data-based methods fine-tune the LLM using a set of modified responses. This approach often begins by generating altered outputs (e.g., refusal-based responses), such as obliterated responses~\cite{choi2024snap}, inverted facts~\cite{gu2024meow}, or in-domain plausible alternatives~\cite{mekala2024alternate}. These generated responses are then used to guide the unlearning process. \cite{mekala2024alternate} propose Alternate Preference Optimization, which utilizes in-domain positive feedback on the forget set, complementing the usual negative feedback to overcome the limitations of relying solely on negative feedback during unlearning. In this work, we employ reject-based template outputs as the modified "good" responses for the forgotten samples.

\paragraph{Input-based Methods}
Input-based methods craft input instructions~\cite{pawelczyk2023context,muresanu2024unlearnable,thaker2024guardrail,bhaila2024soft,gao2024practical,liu2024large}, such as in-context examples and prompts, to steer the original LLM toward the unlearning objective without altering the model's parameters. These approaches aim to achieve unlearning in the output space rather than in the parameter space. Among these methods, a notable baseline by~\cite{liu2024large} uses an external prompt classifier as a guardrail, applying embedding corruptions to the identified prompts. The authors demonstrate that this corruption scheme results in distribution-wise similarity to the retrained model.

In this work, we propose a novel loss adjustment method for LLM unlearning, which simultaneously utilizes available example responses, effectively combining data-based and model-based methods.

\subsection{Machine Unlearning} 
In response to the data regulation requirements~\cite{hoofnagle2019european}, machine unlearning (MU) has emerged as a critical process to remove the influence of specific data points, data classes, or even higher-level data concepts from a trained machine-learning model. One direct unlearning method involves retraining the model from scratch after removing the forgotten data from the original dataset, which is often considered the gold standard~\cite{liu2024model, fan2024challenging}. However, this approach comes with significant computational demands. To alleviate this, most research focuses on developing approximate but much faster unlearning techniques, including gradient ascent~\cite{thudi2022unrolling,graves2021amnesiac}, influence unlearning~\cite{izzo2021approximate, warnecke2021machine,wu2022puma}, Fisher forgetting~\cite{becker2022evaluating,golatkar2020eternal}, finetuning-based approaches~\cite{liu2024model,fan2023salun}, and loss correction-related unlearning~\cite{adolphs2022cringe,wang2023kga, di2024label}.



==> LLM_Unlearning_arxiv/src/03-preliminary.tex <==

\section{Preliminaries}
In this section, we introduce the preliminary formulation of LLM unlearning and the existing LLM unlearning framework.

\subsection{Formulation}
Given a forget dataset $D_f$, a retain dataset $D_r$, and an LLM $\theta_o$, the task of LLM unlearning is to fine-tune the original model such that the updated LLM $\theta$ resembles a model trained without $ D_f$.

For a prompt-response pair $(x,y)$, the loss function on $y$ for fine-tuning is $\mathcal{L}(x,y;\theta)=\sum_{i=1}^{|y|} \ell(h_{\theta}(x, y_{<i}),y_i)$, where $\ell(\cdot)$ is the cross-entropy loss, and $h_{\theta}(x, y_{<i}):=\mathbb{P}(y_i|(x, y_{<i}); \theta)$ is the predicted probability of the token $y_i$ given by an LLM $\theta$, with the input prompt $x$ and the already generated tokens $y_{<i}:=[y_1, ..., y_{i-1}]$.

The most straightforward approach to unlearn is Gradient Ascent (GA). GA modifies a trained model so that it "forgets" or minimizes the influence of specific data or patterns it has previously learned. Mathematically, the GA algorithm iteratively updates the model at step $t$ by performing gradient ascent on the next-token prediction loss over the forget dataset: $\theta_{t+1} \leftarrow \theta_t + \lambda \nabla_{\theta_t}\mathcal{L}(x,y;\theta_t)$, where $\lambda$ is the (un)learning rate. 

\subsection{Existing LLM Unlearning Paradigm}
\label{sec:2.2 paradigm}
The mainstream class of existing LLM unlearning methods involves fine-tuning the original LLM against an unlearning objective function. Although the exact designs vary, the general type of loss adjustment in LLM unlearning can be characterized as follows:
\begin{equation}\label{eq:general}
    L = L_{\textbf{FG}} + L_{\textbf{RT}} + L_{\textbf{Custom}}.
\end{equation}

The modified loss function comprises three main components:

\squishlist
    \item \textbf{$L_{\text{FG}}$ (Forget Loss)}: Encourages the model to "forget" the undesired data or patterns. This typically involves increasing the loss on the data to be forgotten, effectively making the model perform worse on those specific examples. The goal is to reduce the model's reliance on these data points, thereby minimizing their influence on future predictions.
    
    \item \textbf{$L_{\text{RT}}$ (Retain Loss)}: Ensures that the model maintains its overall performance and general knowledge on unaffected data. It typically involves using the original loss function from training or a modified version that focuses on the data the model is meant to retain. This term prevents the unlearning process from degrading the model's overall capabilities beyond the scope of the specific unlearning objective.
    
    \item \textbf{$L_{\text{Custom}}$ (Custom Loss)}: Allows for additional flexibility and customization in the unlearning process. It may include regularization terms to control the magnitude of parameter updates or specific constraints to enforce certain unlearning behaviors. This component enables researchers to tailor the unlearning process to specific requirements or incorporate domain-specific knowledge.
\squishend

In summary, common loss adjustment methods employ one~\cite{jang2022knowledge}, two~\cite{liu2022continual, maini2024tofu, zhang2024negative}, or all three~\cite{yao2023large} of these components to guide the model towards forgetting specific data while minimizing the impact on its overall performance and utility. The interplay between these terms allows for controlled and targeted unlearning, ensuring the model retains its valuable capabilities while selectively forgetting undesired information. More detailed formulations of these loss adjustment-based methods, along with related work, are deferred to Appendix~\ref{app:baseline_formulation} and Appendix~\ref{app:related_work}.


\paragraph{An Example: Large Language Model Unlearning (LLMU).} We adopt a popular approach in LLM unlearning, LLMU \cite{yao2023large}, to interpret a special case of Eqn. (\ref{eq:general}). Specifically, the objective of LLMU contains three components: the Unlearn Harm $L_{\textbf{FG}}$, the Maintain Performance $L_{\textbf{RT}}$, and the Random Mismatch $L_{\textbf{Random}}$ (the custom loss). The training objective is as follows:
    $$
        L_{\textbf{LLMU}} = L_{\textbf{FG}} + L_{\textbf{RT}} + L_{\textbf{Random}} ,
    $$
    The forget loss $L_{\textbf{FG}}=-\sum_{(x_f,y_f)\in  D_f} \mathcal{L}(x_f,y_f;\theta) $, where $(x_f, y_f)$ indicates the forget data pairs from the forget dataset $D_f$, $\theta$ is the updated unlearned model. It is actually the Gradient Ascent loss to forget the samples subject to unlearning. 
    The retain loss 
    $L_{\textbf{RT}} = \sum_{(x_r, y_r)\in D_r} \sum_{i=1}^{|y_r|} KL(h_{\theta_o}(x_r,y_{r<i})||h_{\theta}(x_r,y_{r<i}))$, where $KL(\cdot)$ is the KL divergence term, $(x_r, y_r)$ indicates the retain data pairs from the retain dataset $D_r$, $\theta_o$ is the original model, and $\theta$ is the updated model. 
    The random loss $ L_{\textbf{Random}} = \sum_{(x_f, \cdot) \in D_f} \frac{1}{|Y_{rdn}|}\sum_{y_{rdn} \in Y_{rdn}} \mathcal{L}(x_f, y_{rdn}; \theta).
    $ Here, $Y_{rdn}$ is a set of random responses that do not have a connection to the forget prompts $x_f$. 


==> LLM_Unlearning_arxiv/src/04-method.tex <==

\section{Method}
\input{tables/divergence}
In this section, we introduce \textbf{F}orget data only \textbf{L}oss \textbf{A}justmen\textbf{T} (\textbf{FLAT}), a "flat" loss adjustment approach which adjusts the loss function using only the forget data, by leveraging $f$-divergence maximization towards the distance between the preferred template and original forget responses. 
We first derive the formulation of our method via $f$-divergence maximization (\S~\ref{sec: 4.1_diver_max}), followed by the presentation of the empirical alternative to our approach (\S~\ref{sec:4.2_empiraical}). In section \S~\ref{sec:4.3_upper_bound}, we explore the estimation gap between the theoretical and empirical $f$-divergence. Finally, we discuss the connection between our method and DPO (\S~\ref{sec:4.4_dpo}).


\subsection{Loss-Adjustments via $f$-divergence Maximization}
\label{sec: 4.1_diver_max}


For each learning batch, we assume that we only have access to a set of forget samples $(x_f,y_f) \in D_f$. Instead of directly adopting gradient ascent over these forget samples, we propose to maximize the divergence between exemplary and bad generations of forget data. Key steps are summarized as below.


\squishlist
    \item \textbf{Step 1:} Equip example/template responses $y_e$ for each forget sample $x_f$. Together we denote the paired samples as $ D_e = \{(x_{f}^j, y_{e}^j)\}_{j\in[N]}$. 

    This could be done by leveraging open-source LLMs such as Llama 3.1 \cite{dubey2024llama}
    or self-defining the responses according to our wish, etc. The designated unlearning response could be a reject-based answer such as "I don’t know" (denoted as "IDK") or an irrelevant answer devoid of the unlearning target-related information. 
    
    \textbf{Motivation:} Step 1 generates example responses for LLM fine-tuning and provides better instructions on what LLM should respond given the forget data. Besides, certain existing methods make LLM generate hallucinated responses after unlearning, which further illustrates the importance of example responses for LLM unlearning.
    \item \textbf{Step 2:} Loss adjustmens w.r.t. the sample pairs $(x_f, y_e, y_f)$ through:
    \begin{align}\label{eqn:format}
        L(x_f,y_e, y_f;\theta)=\lambda_e \cdot L_e(x_f,y_e;\theta) - \lambda_f \cdot L_f(x_f, y_f;\theta),
    \end{align}
    where $L_e, L_f$ are losses designed for the data sample $(x_f, y_e)$ and $(x_f, y_f)$, respectively. The corresponding closed form will be introduced in Section \S~\ref{sec:4.2_empiraical}.
    
    \textbf{Motivation:} Step 2 encourages the LLM to forget the forget data with bad responses, meanwhile, learn to generate good responses on relevant forget data. [such as template answers]
    \item \textbf{Step 3:} How to decide on the values of $\lambda_e$ and $\lambda_f$? 

    We leverage $f$-divergence to illustrate the appropriate balancing between $L_e(x_f,y_e;\theta)$ and $L_f(x_f, y_f;\theta)$. Assume  $x_f, y_e$ is generated by the random variable $X_f, Y_e$ jointly following the distribution $ \mathcal D_e$. Similarly, $x_f, y_f$ is given by $X_f, Y_f$ and $(X_f, Y_f)\sim \mathcal D_f$.
    Step 2 shares similar insights as if we are maximizing the divergence between $\mathcal D_e$ and $ \mathcal D_f$. 
    Our theoretical purpose is to obtain the model that maximizes the $f$-divergence between $\mathcal D_e$ and $\mathcal D_f$, defined as $f_{div} (\mathcal D_e || \mathcal D_f)$. 


\paragraph{The variational form $f$-divergence}

% Now the objective function becomes: $ L(X, Y_u, Y_e; \theta)=f_{div} (D_u || D_e)$. 
Instead of optimizing the $f_{div} $ term directly, we resolve to the variational form of it. 
Due to the Fenchel duality, we would have:
\begin{align}\label{eqn:fdiv}
    % \theta^*&:=\arg \max_{\theta} D_f (D^G || D^U)\\
    f_{div} (\mathcal D_e || \mathcal D_f)=\sup_{g}\left[ \mathbb{E}_{\mathcal{Z}_e \sim \mathcal D_e}\left[ g(\mathcal{Z}_e)\right] - \mathbb{E}_{\mathcal{Z}_f \sim \mathcal D_f}\left[ f^*(g(\mathcal{Z}_f))\right]\right]:= \sup_{g} \text{VA}(\theta, g),
\end{align}
we define $f^*$ as the conjugate function of the $f$-divergence function. For simplicity, we define $\text{VA}(\theta, g^*):=\sup_{g} \text{VA}(\theta, g)$, where $g^*$ is the optimal variational function. 

Hence, the objective of \method is to obtain: $\theta^* := \arg \max_{\theta} \text{VA}(\theta, g^*)$. 

\textbf{Motivation:} Note that existing solutions fail to keep a good balance between model performance on forget data and retain data, step 3 provides a formal theoretical framework of our loss revision in Step 2, under the $f-$divergence maximization between $\mathcal D_e$ and $ \mathcal D_f$, the method assigns the appropriate weights $f^*(\cdot), g^*(f^*(\cdot))$ w.r.t. the joint data distributions $\mathcal D_e, \mathcal D_f$.  
\squishend
% \begin{align*}
%     \theta^* := \arg \max_{\theta} \text{VA}(\theta, g^*)
% \end{align*}


% \paragraph{Motivation:}
% \squishlist
%     \item Step 1 generates good samples for LLM fine-tuning, provides better instructions on what LLM should respond given toxic/forget data.
%     \item Step 2 contrastively encourages the LLM to forget on forget data with bad response, meanwhile, learn to generate good response on relevant forget data. [could be either blank answer, or template good answers]
%     \item Note that existing solutions fail to keep a good balance between model performance on forget data and retain data, step 3 provides a formal theoretical framework of our loss revision in Step 2, under the $f-$divergence maximization between two properly defined divergence $D^G, D^U$, the method assigns the appropriate weights $\lambda_e, \lambda_U$ to be $f^*(\cdot), g^*(f^*(\cdot))$, in the view of $f$-divergence.  
% \squishend

\subsection{Empirical Alternative of Loss Adjustment}
\label{sec:4.2_empiraical}
% \paragraph{Loss Adjustment format}
Note that Eqn. (\ref{eqn:fdiv}) could be viewed as a data distribution level loss adjustment, 
% hence, the closed form of Eqn. (\ref{eqn:format}) can be denoted by:
  % \begin{align}\label{eqn:la}
  %       L(x_u,y_e, y_u;\theta)=g^*(\mathbb{P}(x_u,y_e;\theta)) - f^*(g^*( \mathbb{P}(x_u,y_u;\theta))),
    % \end{align}
in practice, when given access to a set of forget data as well as example and bad answers, $x_f,y_e, y_f$, the per-sample loss function (closed form of Eqn. (\ref{eqn:format})) would be given by\footnote{To clarify, we introduce the negative sign on the r.h.s. because loss function is commonly combined with the minimization task, while our method is formulated as maximizing the $f$-divergence.}:
    \begin{align}\label{eqn:larsf}
        L(x_f,y_e, y_f; \theta)&= -\left[\sup_{g} \left[ g(\mathbb{P}(x_f,y_e;\theta)) - f^*(g( \mathbb{P}(x_f,y_f;\theta)))\right]\right]\notag\\&= -g^*(\mathbb{P}(x_f,y_e;\theta)) + f^*(g^*( \mathbb{P}(x_f,y_f;\theta))).
    \end{align}
We provide examples of $f$-divergence functions in Table \ref{table:f_div}, along with their conjugate and variational functions \cite{nowozin2016f,wei2021when}. We illustrate via following examples.
% \wjh{TODO for myself: unify the max/min}
% \input{tables/method_f_divergence}

\paragraph{Example 1: Total-Variation}

For Total-Variation (TV), an example of $f$-divergence, $f^*(u)=u, g^*(v)=\frac{\tanh{(v)}}{2}$, hence, {\small$g^*(\pg) - f^*(g^*(\pu)=\frac{\tanh{(\pg)}}{2}-\frac{\tanh{(\pu)}}{2}.$}
% \begin{align*}
%     g(\pg) - f^*(g(\pu)
%     &=\frac{\tanh{(\pg)}}{2}-\frac{\tanh{(\pu)}}{2}.
% \end{align*}
We defer examples of other $f$-divergence functions in the Appendix \ref{app:eg}.

% where
\paragraph{How to estimate $\pg, \pu$?}
\ \
% Empirically, in light of \cite{yao2023large}, 
% we define $h_{\theta}(x, y_{<j}):=\mathbb{P}(y_j|(x, y_{<j}); \theta)$ be the predicted probability of the token $y_j$ given by an LLM $h_\theta$, with the input prompt $x$ and the generated tokens $y_{<j}:=[y_1, ..., y_{j-1}]$. # already in section 2.
% we estimate $\pg, \pu$ via the following two quantities: $$\mathbb{P}(x_u,y_e;\theta):=\frac{\sum_{i=1}^{|y_e|} \mathbb{P}(h_{\theta}(x_i^U, {y_i^G}_{<j})={y_i^G}_j)}{|y_i^G|}, \quad \mathbb{P}(x_i^U,y_i^U;\theta):=\frac{\sum_{j=1}^{|y_i^U|} \mathbb{P}(h_{\theta}(x_i^U, {y_i^U}_{<j})={y_i^U}_j)}{|y_i^G|}.$$
We define the following two quantities: $$\mathbb{P}(x_f,y_e;\theta):=\frac{\sum_{i=1}^{|y_e|} P(h_{\theta}(x_f, y_{e,<i})=y_{e,i})}{|y_e|}, \quad \mathbb{P}(x_f,y_f;\theta):=\frac{\sum_{i=1}^{|y_f|} P(h_{\theta}(x_f, {y_{f,<i}})=y_{f,i})}{|y_f|}.$$
% \wyx{TODO:change the notation of P to $L_e$ and $L_f$}

Here, $y_{e,i}$ and $y_{f,i}$ denote the $i$-th token in the samples $y_e$ and $y_f$, respectively, while ${y_{e,<i}}$ and ${y_{f,<i}}$ represent the already generated tokens. $|y_e|$ and $|y_f|$ are the lengths of the example response $y_e$ and the forget response $y_f$, respectively. 
Given a prompt and the previously generated tokens, $P(h_{\theta}(x_f, y_{e,<i}) = y_{e,i})$ and $P(h_{\theta}(x_f, {y_{f,<i}}) = y_{f,i})$ are the probabilities of correctly predicting the next token. These two quantities represent the average probabilities of correctly generating tokens for the template and forget responses, respectively. 
% \wjh{add more explanations how these quantities}\wyx{solved} 
To align Eqn. (\ref{eqn:larsf}) with Eqn. (\ref{eqn:format}), we could define $\lambda_e=\lambda_f=1$, $L_e(x_f,y_e;\theta):= -g^*(\mathbb{P}(x_f,y_e;\theta))$, and $L_f(x_f,y_f;\theta):= -f^*\left(g^*(\mathbb{P}(x_f,y_f;\theta))\right)$.


    

\subsection{The upper bound of the estimation gap}
\label{sec:4.3_upper_bound}
% \wjh{TODO for myself: check notations are well defined and add proof in the appendix}
To connect the empirical alternative of \method with the corresponding theoretical format, in this section, we aim to explore the estimation gap between the theoretical $f$-divergence $f_{div} (\mathcal D_e || \mathcal D_f)$ and the empirical optimal estimated $f$-divergence $\hat{f}_{div} (D_e || D_f)$, here we define:
\begin{align*}
    \hat{f}_{div} (D_e || D_f):= \mathbb{E}_{{Z}_e \sim D_e}[ \hat{g}({Z}_e)] - \mathbb{E}_{{Z}_f \sim D_f} [f^*(\hat{g}({Z}_f))],
\end{align*}
where $\hat{g}:=\sup_{g\in \Phi} \mathbb{E}_{{Z}_e \sim D_e}[ g({Z}_e)] - \mathbb{E}_{{Z}_f \sim D_f} [f^*(g({Z}_f))]$ and $\Phi$ is the function space.

% \paragraph{Preliminary}

\begin{assumption}[Bounded Density Ratio]\label{ass:bdr}
    The density ratio ${Z}_e/{Z}_f$ is lower and upper bounded by positive constants $a$ and $b$, respectively.
\end{assumption}
Assumption \ref{ass:bdr} is wildely adopted by the literature \cite{suzuki2008approximating,nguyen2010estimating}, which necessitates that the probability density functions ${Z}_e, {Z}_f$ share the same support.
\begin{assumption}[Regularity of Divergence Function]\label{ass:rdf}
$f(\cdot)$ is smooth on $[a, b]$, and $f(1)=0$. $f$ is $\mu_0$-strongly convex, and has $L_0$-Lipschitz continuous gradient on $[a, b]$, for positive constants $\mu_0, L_0$.
\end{assumption}
Assumption \ref{ass:rdf} is a mild condition since it only requires the condition to hold for the interval $[a, b]$, which works for many commonly used $f$-divergence functions, i.e., KL divergence.
% \begin{definition}[Covering Number]

Let $(V, ||\cdot||_{L_2})$ be a normed space, and $\Phi\subset V$. ${v_1, ..., v_C}$ is a $\delta$-covering over $\Phi$ of size $C$ if $\Phi \subset \cup_{i=1}^C B(v_i, \delta)$ where $B(v_i, \delta)$ is the $\delta$-ball centered at $v_i$. The covering number is then defined as $C_2(\delta, \Phi)=\min \{C: \exists \delta\text{-covering over } \Phi\text{ of size }C\}$. The following assumption would characterize the representation power of the function space $\Phi$.
% \end{definition}

\begin{assumption}[Order of Covering Number]\label{ass:ocn}
$C_2(\delta, \Phi)=\mathcal{O}(\exp\{\delta^{-r_{\Phi}}\})$, and $r_{\Phi}\in (0, 2)$.
\end{assumption}

\begin{theorem}\label{theorem}
    Given Assumptions \ref{ass:bdr}-\ref{ass:ocn}, suppose $\hat{g}\in \Phi$, with probability $\geq 1-e^{-N^{r_{\Phi}/(2+r_{\Phi})}}$, we have: $\left|\hat{f}_{div} (D_e || D_f) - f_{div} (\mathcal D_e || \mathcal D_f)\right| \precsim N^{-\frac{1}{r_{\Phi}+2}},$ where we have defined $N$ as the number of samples in the forget data.
\end{theorem}
Theorem \ref{theorem} illustrates that the empirical alternative of \textbf{FLAT}, $\hat{f}_{div} (D_e || D_f) $, achieves the optimal non-parametric rate of convergence towards $f_{div} (\mathcal D_e || \mathcal D_f)$.
\subsection{Connection with DPO}
\label{sec:4.4_dpo}
In this section, we discuss the connection and key differences between our approach and the celebrated Direct Preference Optimization (DPO) \cite{rafailov2024direct} approach for aligning LLMs. 

Given a dataset $ D={\{(x_{f}^j, y_{e}^j, y_{f}^j)\}}_{j \in [N]}$, where $y_e$ and $y_f$ are preferred template and original forget responses to the forget prompt $x_f$, DPO~\cite{rafailov2024direct} fine-tunes original model $\theta_o$ using $ D $ to better align it with good answer preferences, which minimizes:
% {\small
{
    \begin{align*}
        L_{\textbf{DPO},\beta}(\theta) &= -\frac{2}{\beta} 
\E_{D}\Big[ \log  \sigma \Big( \beta \log \frac{\pi_\theta(y_e\mid x_f)}{\pi_{ref}(y_e \mid x_f)} - \beta  \log \frac{\pi_\theta(y_f\mid x_f)}{\pi_{ref}(y_f \mid x_f)}\Big) \Big] \\&= -\frac{2}{\beta} 
\E_{D} \Big[ \textcolor{red}{\log  \sigma \Big ( \beta (\log \prod_{i=1}^{|y_e|}} h_\theta(x_f, y_{e,<i}) - \textcolor{red}{\log \prod_{i=1}^{|y_f|}} h_\theta(x_f, y_{f,<i})) \textcolor{red}{- M_{ref} \Big)} \Big],
    \end{align*}}
where, $\sigma(t)=\frac{1}{1+e^{-t}} $ is the sigmoid function, $\beta > 0$ is the inverse temperature, $\pi_\theta := \prod_{i=1}^{|y|} h_{\theta}(x, y_{<i})$ is the predicted probability of the response $y$ to prompt $x$ given by LLM $\theta$, $\pi_{ref}$ is the predicted probability given by reference model, and $M_{ref} := \beta (\log \prod_{i=1}^{|y_e|} h_{\theta_o}(x_f, y_{e,i}) - \log \prod_{i=1}^{|y_f|} h_{\theta_o}(x_f, y_{f,i}))$.  

As for \textbf{FLAT}, we calculate the average probability of all correctly generated tokens and employ a novel re-weighting mechanism that assigns different importance to each term using distinct activate functions for both the example and forget loss terms, which minimizes:
{\begin{align*}
    L_{\textrm{\textbf{FLAT}}}(\theta) &= - \E_{D} \Big[  \textcolor{red}{g^*( \frac{1}{|y_e|} \sum_{i=1}^{|y_e|} }h_{\theta}(x_f, y_{e,<i})\textcolor{red}{)} - \textcolor{red}{f^*(g^*( \frac{1}{|y_f|} \sum_{i=1}^{|y_f|} }h_{\theta}(x_f, y_{f,<i}) \textcolor{red}{)} \Big].
\end{align*}}
Here, $f^*(\cdot), g^*(f^*(\cdot))$ are the activate functions that assign appropriate weights to each loss term. The detailed derivation is in Appendix~\ref{app:derivation}. The key differences are highlighted in \textcolor{red}{red}.
% \paragraph{Example 2: KL}
% For KL f-divergence, $f^*(u)=e^{u-1}, g_f(v)=v$, hence, {\small$ g(\pg) - f^*(g(\pu)=\pg-e^{\pu-1}.$} 
% Here, $\mathbb{P}(x_f,y_e;\theta)$ and $\mathbb{P}(x_f,y_f;\theta)$ are defined in Section~\S~\ref{sec:4.2_empiraical}
   % \wyx{Currently working on the derivation of the empirical loss} 
% \yang{this equation is out of place. and its better to recap our formula here and compare the key differences using coloring} \wyx{add our loss function}
Specifically, DPO relies on a reference model to guide the unlearning process, whereas \method only uses a sample pair dataset containing both exemplar and forget responses. Besides, our solution differs from DPO in three critical aspects: the re-weighting activation function, whether to sum or average the token losses, and whether to apply the logarithm to the output probability. 
We conduct an ablation study with DPO to evaluate the effectiveness of the proposed re-weighting mechanism in Section~\S~\ref{sec:ab}.


==> LLM_Unlearning_arxiv/src/05-exp.tex <==

\section{Experiment}
% @Yaxuan
In this section, we compare the proposed method with baseline unlearning methods on three widely used LLM unlearning tasks: copyrighted content unlearning on Harry Potter (HP) Series Book~\cite{yao2023large} (\S ~\ref{copyright}), entity unlearning on TOFU dataset~\cite{maini2024tofu}  (\S ~\ref{entity}), and unlearning on MUSE-News benchmark~\cite{shi2024muse}  (\S ~\ref{muse}). We conduct additional ablation studies to assess the effectiveness of our methods in Section \S~\ref{sec:ab}.



\subsection{Baseline Methods}
\label{sec:baseline}
We evaluate the effectiveness of our proposed method \method by comparing it to a series of strong LLM unlearning baselines, particularly those based on loss adjustment. 
We consider Gradient Ascent (GA)~\cite{jang2022knowledge,yao2023large}, KL minimization (KL)~\cite{maini2024tofu}, GradDiff (GD)~\cite{liu2022continual}, and NPO~\cite{zhang2024negative} across all three tasks. 
For copyrighted content and entity unlearning, we also include Preference Optimization (PO)~\cite{maini2024tofu}, Large Language Model Unlearning (LLMU)~\cite{yao2023large}, and DPO~\cite{rafailov2024direct}.
For the Harry Potter dataset, we add Mismatch~\cite{liu2024large} as a simple and effective baseline method.
For the MUSE-News benchmark, we additionally consider Task Vectors~\cite{ilharco2022editing}, Who's Harry Potter (WHP)~\cite{eldan2023s} and an extended version of NPO (NPO-RT) as a comparable method, which incorporates a fine-tuning term on the retain dataset.
Further experiment details are provided in Appendix~\ref{app:baseline_formulation}.




\subsection{Copyrighted Content Unlearning}
\label{copyright}

\textbf{Experiment Setup.} 
We select Harry Potter and the Sorcerer's Stone~\cite{rowling1997harry} as the copyrighted content for unlearning. The objective is to ensure that the unlearned model does not generate passages with high similarity to the original text.
Following prior works~\cite{liu2024large, yao2023large}, we first fine-tune LLMs on the corresponding corpus, treating it as the model subject to unlearning, while using the original pre-trained checkpoint as the retained model\footnote{We empirically verified that the initial LLM cannot generate the original corpus, making it a valid candidate for retrained model.}.
Following~\cite{yao2023large,jia2024soul}, We extract 400 chunks from the Harry Potter book series dataset~\cite{eldan2023s}, with each chunk containing up to 512 tokens, to create the forget dataset $D_f$. We sample 400 paragraphs in the C4 dataset~\cite{raffel2020exploring} as the retain data $D_r $. The IDK dataset comes from~\cite{jia2024soul}.
We experiment with OPT-2.7B~\cite{zhang2022opt} and Llama2-7B~\cite{touvron2023llama} for this task.

\textbf{Evaluation Metrics.} We report three key metrics to assess the unlearning efficiency and model utility of the unlearned models.
For unlearning efficiency, we use the Forget Quality Gap (FQ Gap), similar to~\cite{liu2024large}, which is the sum of the BLEU Gap and ROUGE-L Gap. It is the absolute difference between the retained model and the unlearned model on these metrics. Specifically, we calculate BLEU~\cite{papineni2002bleu} and ROUGE-L~\cite{lin2004rouge} scores by comparing ground-truth excerpts with completions generated by the unlearned model, given a fixed prefix length of 200 tokens from the forget data, to reflect potential copyright content leakage. We further conduct study on the prompt length for evaluation in Appendix~\ref{app-sec:resuls_hp}. Note that for these metrics, values closer to those of the retained model indicate better unlearning, while values that are too large or too small suggest a difference from the retained model~\cite{liu2024large}.
Following~\cite{ji2024reversing}, we measure the model utility using the zero-shot accuracy on nine standard LLM benchmarks to determine if the generated text remains meaningful and diverse. Additionally, we measure perplexity (PPL) on Wikitext~\cite{merity2016pointer}. More details about the experimental setup and implementation  are in Appendix~\ref{app:hp-setting}.

\textbf{\method consistently ranks in the top two across three metrics.} 
Table~\ref{tab:opt27b-hp-main} shows that \textbf{FLAT} ranks in the top two across the three primary metrics, with particularly strong performance in KL f-divergence function. Our method achieves scores close to those of the retained model in terms of the average accuracy across nine LLM benchmarks. 

\textbf{\method approach achieves good trade-off.} 
Our method demonstrates strong unlearning efficiency while preserving model utility as shown in Table~\ref{tab:opt27b-hp-main}.
Although NPO demonstrates the best forget quality, outperforming our method, it severely suffers from lower model utility, as reflected by its PPL score. PO, while also using example responses, has the highest PPL and a weak forgetting performance (FQ Gap), indicating the ineffectiveness of learning the example responses in a naive manner. 
These results highlight the effectiveness of our method in balancing forget quality and model utility, even without an explicit retaining term in the loss function. We also include additional results using Llama 2 (Table~\ref{app-tab:llama2-7b-hp-main}) in Appendix~\ref{app-sec:resuls_hp}.

\input{tables/HP_main}

\subsection{Entity Unlearning}
\label{entity}

\textbf{Experiment Setup.} The TOFU dataset~\cite{maini2024tofu} is a synthetic question-answering dataset focused on author biographies, aiming to enable a LLM to unlearn a portion of fictitious authors while retaining knowledge about the rest and real-world facts. The dataset includes 200 fake authors, each with 20 QA pairs, and experiments are conducted with 1\% of these authors marked for unlearning.
We use Llama2-7B~\cite{touvron2023llama}, Phi-1.5B~\cite{li2023textbooks}, and OPT-2.7B~\cite{zhang2022opt} as base LLM.

\textbf{Evaluation Metrics.} 
To assess forget quality and model utility, we mainly use two metrics proposed alongside the TOFU dataset, Forget Quality (FQ) and Model Utility (MU)~\cite{maini2024tofu}. Forget quality, assessed via a p-value from a Kolmogorov-Smirnov test, measures how closely the unlearned model's output matches a model trained only on the retained data in distribution. When the p-value is above 0.01, we say the forgetting is significant. Model utility is the aggregated model performance on held-out retain data regarding fictional authors, real-world author profiles, and world facts. We also report the ROUGE-L score on forget set and retain set. 
It's important to note that for the forget set, a lower ROUGE-L score does not necessarily indicate better performance. Therefore, we highlight methods where the ROUGE-L score closely matches that of the retained model, as these are considered to produce better results.
More metrics can be found in Appendix~\ref{app:tofu_eval_metrics}.



\textbf{\method is always the best in preserving model utility.} As seen in Table~\ref{tab:tofu-main}, it experiences almost no reductions in model utility compared to the original model. On LLaMA2-7B, although GA and KL achieve strong ROUGE-L scores on the retain dataset, their forgetting performance is poor. Similarly, on Phi-1.5B, GD performs well on the retain dataset’s ROUGE-L score, but its forgetting performance is insufficient, failing to exceed 0.01. 
 
 \textbf{\method achieves the top two Forget Quality under all three models.} \textbf{FLAT} achieves a ROUGE score that is closest to the Retained LLM on forget dataset under Llama2-7B and Phi-1.5B. PO shows the best forgetting efficiency on Phi-1.5B, but its ROUGE-L scores on both the forget and retain datasets are lower compared to the retained LLM, indicating weaker model utility. A similar issue is observed with GA: while it excels in forgetting performance on the OPT-2.7B model, its model utility remains weaker.

\textbf{\method achieves the best trade-off.}
Our method consistently ranks in the top two across the primary metrics, achieving the best performance in MU. Specifically, KL f-divergence demonstrates strong results in both FQ and MU on LLama2-7B and Phi-1.5B models. Overall, all four f-divergence functions effectively balance forgetting efficiency and model utility.
In summary, our method demonstrates the best model utility while achieving top-two results in forgetting performance.


\input{tables/TOFU_main}
\subsection{MUSE-News Unlearning}
\label{muse}
\textbf{Experiment Setup.}
We focus on the task of unlearning on News corpus presented in~\cite{shi2024muse}. News consists of BBC news articles~\cite{li2023avoiding} collected after August 2023. All articles are randomly divided into forget, retain, and holdout sets.
We perform unlearning directly on the pre-trained models provided by the benchmark, following the corresponding experimental setup.

\textbf{Evaluation Metrics.} We report the proposed four metrics, \textit{VerbMem} on forget dataset, \textit{KnowMem} on forget and retain dataset, and Privacy leakage (\textit{PrivLeak}). We quantify the verbatim memorization \textit{VerbMem} by prompting the model with the first l tokens from a sequence and comparing the continuation outputted by the model $\theta$ to the true continuation using the ROUGE-L F1 score~\cite{lin2004rouge}. We gather the model's answers to questions and then average the ROUGE scores for all question-answer pairs in forget dataset or retain dataset to compute the knowledge memorization score \textit{KnowMem}.
The \textit{PrivLeak} metric for a good unlearning algorithm should be close to zero, whereas an over/under-unlearning algorithm will get a large positive/negative metric. 

\input{tables/MUSE_main}

\textbf{Experiment Results.} \method effectively removes verbatim and knowledge memorization of forget dataset and achieve good knowledge memorization of retain dataset. But it can still reveal the membership of $D_f$ in $D_r$.
As shown in Table~\ref{tab:llama2-7b-muse}, GA, NPO, GD, WHP, and ours perform well in VerbMem and KnowMem on forget dataset, often reduing them even beyond the levels achieved by the retrained model. However, these reductions often come at the cost of significant utility loss on the retain set. Only GD, WHP and ours can perfome good in all memorization related metrics. And \method(TV) can achieve the lowest VerbMem and KnowMem on $D_f$ and the highest KnowMem on $D_r$ among the three methods. However, none of the methods can achieve satisiable results regarding to the privacy leakage. Since MUSE uses news data, which is highly time-dependent (and thus possibly non-i.i.d.), we advocate for cautious interpretation of the PrivLeak metric. A detailed analysis is provided in Appendix~\ref{app:muse_evaluation_metrics}.




\subsection{Ablation Studies}
\label{sec:ab}


\textbf{The Effectiveness of Re-weighting Mechanism.} As \method(KL) demonstrates strong overall performance, we base our ablation study on KL divergence to explore the effectiveness of the implicit re-weighting mechanism within our loss adjustment. This study is conducted on the TOFU dataset using Llama2-7B. For the ablation study on the HP dataset, please refer to Table~\ref{app-tab:llama2-7b-hp-ab-reweighting} in Appendix~\ref{app:ab_study}.

When using preferred template data for unlearning, we compare our method with DPO (without the term $M_{ref}$) and SimPO, as outlined in Appendix~\ref{app:baseline_formulation}. All methods use the same data and have similar formulations, with two terms in the loss function; the only difference lies in the intrinsic re-weighting mechanism.  As shown in Table~\ref{tab:ab_re_tofu}, our method achieves the highest number of best results across 12 metrics. When replacing the IDK data with retain data, the results show that the retain version performs better on the Retain Set but worse on Real Authors and Real World compared to \method(KL). 

Since GD shares the same data usage and formulation as our method, except for the re-weighting mechanism and utilization of retain data, we compare the retain version to GD. The results show that our method achieves better performance on both the Retain Set and Forget Set, with the decline in Real Authors and Real World performance caused by the use of retain data.


\input{tables/ab-reweight}



\textbf{The Imapct of Good Answer Type.} In the first step of our approach, we intend to generate good example responses for each forget sample. We primarily use the reject-based response "I don't know" (denoted as IDK) as the default choice. In this section, we conduct an ablation study on data usage for \textbf{FLAT} to analyze how these good responses impact unlearning performance. 
Table~\ref{tab:tofu-llama2-ab-answer_type} presents the ablation study of good answer type using three LLMs on TOFU dataset, comparing IDK with random normal responses (denoted as Normal). Table~\ref{app-tab:llama2-7b-hp-ab} in Appendix~\ref{app:ab_study} provides the ablation study of different good answer type using Llama2-7B on the HP dataset. Results indicate that using normal responses improves model utility on HP datasets and improves ROUGE-L Score on retain set on TOFU datasets, whereas using IDK responses yields better forgetting quality. 

Additionally, we observe that the performance across the four divergence functions is relatively similar. 
KL divergence, in particular, demonstrates more consistent results across the three datasets and three models, likely due to its reduced sensitivity to incorrect or bad answers.

\input{tables/ab_study}

==> LLM_Unlearning_arxiv/src/06-conclusion.tex <==
\section{Conclusion}
In this paper, we address the limitations of existing LLM unlearning methods, which often rely on the retain data or a reference LLM for response calibration. To overcome these challenges, we propose \method (Forget data only Loss AdjustmenT), a "flat" loss adjustment approach that eliminates the need for retain data or a reference model. By optimizing the $f$-divergence between the template and forget responses, \method offers a clear and theoretically grounded solution for balancing forget quality with model utility in LLM unlearning. Through extensive experiments on three key unlearning tasks: copyrighted content unlearning on the Harry Potter dataset, the MUSE benchmark, and entity unlearning on the TOFU dataset, we demonstrate the superior performance of \textbf{FLAT}. Our method consistently achieves high unlearning efficiency while preserving overall model utility, showcasing its effectiveness in addressing both practical and theoretical challenges in LLM unlearning.





==> LLM_Unlearning_arxiv/tables/HP_main.tex <==
% \begin{wraptable}{r}{0.45\linewidth}  
\begin{table}[htb]
\centering
% \vspace{-0.15in}
\caption{Performance of our method and the baseline methods on Harry Potter dataset using OPT-2.7B. \method consistently ranks in the top two in terms of similarity to the retained model, measured by Forget Quality Gap (FQ Gap), while also generating meaningful and diverse outputs, as reflected by perplexity (PPL) and the average zero-shot accuracy across nine LLM benchmarks (Avg. Acc.). The top two results across three main metrics are highlighted in  \highlight[cyan!20]{\textbf{blue}}.}
% \vspace{-3mm}
\resizebox{0.56\linewidth}{!}{
\begin{tabular}{c|ccc}
\toprule
\textbf{Metric} & \multicolumn{1}{c}{\textbf{FQ Gap(\(\downarrow\))}} & \multicolumn{1}{c}{\textbf{PPL(\(\downarrow\))}}& \multicolumn{1}{c}{\textbf{Avg.Acc.(\(\uparrow\))}}  \\ 
\midrule
Original LLM  & 1.5346 & 15.6314 & 0.4762\\
Retained LLM  & 0.0 & 14.3190  & 0.4686  \\
\midrule
GA &  2.7301 & 1.0984e71  & 0.3667  \\
KL & 2.7301 & 16.1592  & 0.4688 \\
GD & 2.3439 & 16.1972  & 0.4690\\
PO & 2.1601 & \colorbox{cyan!20}{\textbf{14.8960}} & 0.4583  \\ 
Mismatch & 1.4042 & 15.7507 & 0.4679 \\
\midrule
LLMU &  2.4639 & 15.8398 & 0.4656 \\ 
DPO & 2.2152 & 16.8396  & 0.4621 \\
NPO  & \colorbox{cyan!20}{\textbf{1.2611}} & 19.6637 & 0.4644 \\
\midrule
\method (TV) &  1.4047 & 15.5512 &  0.4681 \\
\method (KL) &\colorbox{cyan!20}{\textbf{1.3238}} & \colorbox{cyan!20}{\textbf{15.5311}} & \colorbox{cyan!20}{\textbf{0.4694}} \\
\method (JS) & 1.4025 & 15.5499 & \colorbox{cyan!20}{\textbf{0.4693}}\\
\method (Pearson) & 1.4089 & 15.5543 & 0.4686  \\
\bottomrule
\end{tabular}
}
% \vspace{-0.15in}
\label{tab:opt27b-hp-main}
% \end{wraptable}
\end{table}




==> LLM_Unlearning_arxiv/tables/MUSE_main.tex <==
\begin{table}
\caption{Performace on MUSE benchmark using four criteria. We highlight results in \highlight[cyan!20]{\textbf{blue}} if the unlearning algorithm satisfies the criterion and highlight it in \highlight[red!20]{\textbf{red}} otherwise. For metrics on $D_f$, lower values are preferred, while for metrics on $D_r$, higher values are better. In terms of PrivLeak, the results should be close to 0. Large negative or positive values suggest that they may cause privacy leakage. } 
% \vspace{-3mm}
\centering
% \vspace{-2ex}
\resizebox{0.85\textwidth}{!}{
\begin{tabular}{cccccccc}
\toprule
 & \multicolumn{2}{c}{\textbf{VerbMem on $D_f$ (\(\downarrow\))}} & \multicolumn{2}{c}{\textbf{KnowMem on $D_f$ (\(\downarrow\))}} & \multicolumn{2}{c}{\textbf{KnowMem on $D_r$ (\(\uparrow\))}} & \multicolumn{1}{c}{\textbf{PrivLeak}}  \\ 
\midrule
Original LLM  & 58.4 & - & 63.9 & -  & 55.2 & - & -99.8 \\
Retained LLM & 20.8 & - & 33.1 & -  & 55.0 & - & 0.0\\
\midrule
GA & 0.0 &  \colorbox{cyan!20}{(\ding{52})} & 0.0 & \colorbox{cyan!20}{(\ding{52})} & 0.0 & \colorbox{red!20}{(\ding{56})}  & 17.0 \\
KL & 27.4 & \colorbox{red!20}{(\ding{56})}& 50.2 & \colorbox{red!20}{(\ding{56})}& 44.8 & \colorbox{cyan!20}{(\ding{52})}& -96.1 \\
NPO & 0.0 & \colorbox{cyan!20}{(\ding{52})} & 0.0 & \colorbox{cyan!20}{(\ding{52})}& 0.0 & \colorbox{red!20}{(\ding{56})} & 15.0 \\
NPO-RT & 1.2 & \colorbox{cyan!20}{(\ding{52})} &  54.6 & \colorbox{red!20}{(\ding{56})} & 40.5 & \colorbox{cyan!20}{(\ding{52})}  & 105.8 \\
Task Vectors & 56.3 &\colorbox{red!20}{(\ding{56})} & 63.7 & \colorbox{red!20}{(\ding{56})} & 54.6 & \colorbox{cyan!20}{(\ding{52})} & -99.8 \\
\midrule
GD & 4.9 &\colorbox{cyan!20}{(\ding{52})}  & 27.5 & \colorbox{cyan!20}{(\ding{52})} & 6.7 & \colorbox{cyan!20}{(\ding{52})} & 109.4 \\
WHP & 19.7 &\colorbox{cyan!20}{(\ding{52})} & 21.2 & \colorbox{cyan!20}{(\ding{52})} & 28.3 & \colorbox{cyan!20}{(\ding{52})} & 109.6 \\
\midrule
\method (TV) & 1.7 &\colorbox{cyan!20}{(\ding{52})} & 13.6 & \colorbox{cyan!20}{(\ding{52})} & 31.8 & \colorbox{cyan!20}{(\ding{52})} & 45.4\\
\method (KL)  & 0.0 &\colorbox{cyan!20}{(\ding{52})} & 0.0 & \colorbox{cyan!20}{(\ding{52})} &0.0 & \colorbox{red!20}{(\ding{56})} & 58.9  \\
\method (JS) & 1.9 & \colorbox{cyan!20}{(\ding{52})}& 36.2&  \colorbox{red!20}{(\ding{56})}& 38.5 & \colorbox{cyan!20}{(\ding{52})}  & 47.1 \\
\method (Pearson) & 1.6 & \colorbox{cyan!20}{(\ding{52})}& 0.0 &  \colorbox{cyan!20}{(\ding{52})} & 0.2 & \colorbox{cyan!20}{(\ding{52})}  & 26.8 \\
\bottomrule
\end{tabular}
}
\vspace{-0.1in}
\label{tab:llama2-7b-muse}
\end{table}




==> LLM_Unlearning_arxiv/tables/TOFU_main.tex <==
\begin{table}
\caption{Performance of our method and the baseline methods on TOFU dataset using three base LLMs, Llama2-7B, Phi-1.5B, and OPT-2.7B. FQ, MU, R-RL, F-RL represent forget quality, model utility, ROUGE-L on retain dataset and ROUGE-L on forget dataset respectively. We include the original LLM and retain LLM for reference. The top two results are highlighted in \highlight[cyan!20]{\textbf{blue}}.} 
% \vspace{-3mm}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|cccc|cccc|cccc}
\toprule
\textbf{Base LLM} & \multicolumn{4}{c|}{\textbf{Llama2-7B}} & \multicolumn{4}{c|}{\textbf{Phi-1.5B}} & \multicolumn{4}{c}{\textbf{OPT-2.7B}} \\ 
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
\textbf{Metric} & \multicolumn{1}{c}{FQ} & \multicolumn{1}{c}{MU} & \multicolumn{1}{c}{F-RL(\(\downarrow\))} & \multicolumn{1}{c|}{R-RL} & \multicolumn{1}{c}{FQ} & \multicolumn{1}{c}{MU} & \multicolumn{1}{c}{F-RL(\(\downarrow\))} & \multicolumn{1}{c|}{R-RL} & \multicolumn{1}{c}{FQ} & \multicolumn{1}{c}{MU} & \multicolumn{1}{c}{F-RL(\(\downarrow\))} & \multicolumn{1}{c}{R-RL}   \\ 
\midrule
Original LLM & 4.4883e-06 &0.6346  & 0.9851 & 0.9833 & 0.0013 &  0.5184 & 0.9607 & 0.9199 & 0.0013 & 0.5120 & 0.7537 & 0.7494 \\  
Retained LLM & 1.0 & 0.6267 & 0.4080 & 0.9833 & 1.0 & 0.5233 & 0.4272 & 0.9269 & 1.0 & 0.5067 & 0.4217 & 0.7669  \\ 
\midrule
GA & 0.0143 & 0.6333 & 0.4862 &\colorbox{cyan!20}{\textbf{0.9008}} & 0.0013 & 0.5069 & 0.5114 & 0.8048 & \colorbox{cyan!20}{\textbf{0.2657}} & 0.4639 & \colorbox{cyan!20}{\textbf{0.4748}} & 0.6387 \\ 
KL & 0.0068 & 0.6300 & 0.5281 &  \colorbox{cyan!20}{\textbf{0.9398}}& 0.0030 & 0.5047 & 0.5059 & 0.8109 & 0.0286 & 0.4775 & 0.4810 & 0.6613 \\ 
GD & 0.0068 & 0.6320 & 0.4773 & 0.8912 & 0.0030 & 0.5110 & 0.4996 & \colorbox{cyan!20}{\textbf{0.8496}} & 0.0541 & 0.4912 & \colorbox{cyan!20}{\textbf{0.4521}} & 0.6603 \\ 
PO &  \colorbox{cyan!20}{\textbf{0.0541}} & 0.6308& 0.3640  & 0.8811 & \colorbox{cyan!20}{\textbf{0.0286}} & 0.5127 & 0.3170  & 0.7468 & 0.0068 & 0.4424 & 0.0589 & 0.4015 \\  
\midrule
LLMU &  \colorbox{cyan!20}{\textbf{0.0541}} & 0.6337 & 0.4480 & 0.8865 &  \colorbox{cyan!20}{\textbf{0.0286}} & 0.5110 & 0.3058 & 0.7270 &0.0286 & 0.3296 & 0.0347 & 0.2495 \\ 
DPO &  \colorbox{cyan!20}{\textbf{0.0541}} & 0.6359 & 0.5860 & 0.8852 & 0.0521 & 0.0519 & 0.3437 & 0.7349 & 0.0541 & 0.4264 & 0.0806 & 0.3937 \\ 
NPO & 0.0068 & 0.6321 & 0.4632 & 0.8950 & 0.0030 & 0.5057 & 0.5196 & 0.8000 & 0.0541 &  0.4788 & 0.4993 & 0.6490 \\ 
\midrule
\method (TV) & \colorbox{cyan!20}{\textbf{0.0541}}& 0.6373 &  \colorbox{cyan!20}{\textbf{0.4391}} & 0.8826& 0.0143 & \colorbox{cyan!20}{\textbf{0.5168}} & 0.4689 & \colorbox{cyan!20}{\textbf{0.8155}} & 0.0068 &\colorbox{cyan!20}{\textbf{ 0.5086} }& 0.5217 & \colorbox{cyan!20}{\textbf{0.7067}} \\
\method (KL) &  0.0286&  \colorbox{cyan!20}{\textbf{0.6393}} & 0.5199 & 0.8750 &  0.0143 &  \colorbox{cyan!20}{\textbf{0.5180}} &  \colorbox{cyan!20}{\textbf{0.4524}} & 0.7850 & 0.0286 & 0.4838 & 0.4942 & 0.6974 \\
\method (JS) & 0.0541 & 0.6364 & 0.4454 & 0.8864 & 0.0068 & 0.5144  &  \colorbox{cyan!20}{\textbf{0.4572}} & 0.8117 &  \colorbox{cyan!20}{\textbf{0.0541}} &  \colorbox{cyan!20}{\textbf{0.4959}}& 0.4938 & 0.7013 \\
\method (Pearson) & 0.0541 & \colorbox{cyan!20}{\textbf{0.6374}} &  \colorbox{cyan!20}{\textbf{0.4392}} & 0.8857 & 0.0143& 0.5175 & 0.4591 & 0.8099 & 0.0068 & 0.5093 & 0.5052 & \colorbox{cyan!20}{\textbf{0.7059}} \\
\bottomrule
\end{tabular}
}
% \vspace{-0.1in}
\label{tab:tofu-main}
\end{table}

==> LLM_Unlearning_arxiv/tables/ab-reweight.tex <==
\begin{table}
\caption{Ablation Study of Re-weighting Mechanism on TOFU dataset using Llama2-7B under all metrics. We report ROUGE-L score (R-L), Probability (P), and Truth Ratio (TR) on all four subsets of the TOFU benchmark. Higher scores are better except ROUGE-L and Probability on the Forget Set. The best ones are in \highlight[cyan!20]{\textbf{blue}}. }
% \vspace{-3mm}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccc|ccc|ccc|ccc}
\toprule
\textbf{Split} & \multicolumn{3}{c|}{\textbf{Real Authors}} & \multicolumn{3}{c|}{\textbf{Real World}} & \multicolumn{3}{c|}{\textbf{Retain Set}}  & \multicolumn{3}{c}{\textbf{Forget Set}} \\ 
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
\textbf{Metric} & \multicolumn{1}{c}{R-L} & \multicolumn{1}{c}{P} & \multicolumn{1}{c|}{TR} & \multicolumn{1}{c}{R-L} & \multicolumn{1}{c}{P} & \multicolumn{1}{c|}{TR}  & \multicolumn{1}{c}{R-L} & \multicolumn{1}{c}{P} & \multicolumn{1}{c|}{TR} & \multicolumn{1}{c}{R-L(\(\downarrow\))} & \multicolumn{1}{c}{P(\(\downarrow\))} & \multicolumn{1}{c}{TR} \\ 
% \midrule
% Original LLM &  0.9350 & 0.4738 & 0.6210 & 0.8846 & 0.4355 & 0.5579 & 0.9833 & 0.9900 & 0.4662 & 0.9851 & 0.9898 & 0.5123\\  
% Retain LLM & 0.9230 & 0.4645 & 0.6118 & 0.8932 & 0.4182 & 0.5449 & 0.9833 & 0.9902 & 0.4724 & 0.4080 & 0.1798 & 0.6939\\ 
\midrule
 \rowcolor{beaublue!20}
\multicolumn{13}{c}{\textbf{Study on Re-weighting Mechanism Using Template IDK Data}} \\
\midrule
DPO & \colorbox{cyan!20}{\textbf{0.9330}}& 0.4939 & 0.6384 & 0.8917 &  \colorbox{cyan!20}{\textbf{0.4631}} & 0.5646 &  \colorbox{cyan!20}{\textbf{0.8852}} & 0.9623 & 0.4407 & 0.5860 & 0.8734 & 0.6240 \\
DPO w/o $M_{ref}$ & 0.9330 & 0.4899 & 0.6333 & 0.8917 & 0.4620 & 0.5642 & 0.8735 & 0.9579 & 0.4388 &  \colorbox{cyan!20}{\textbf{0.4021}} & 0.8149 & 0.6326\\
SimPO & 0.9330 & 0.4902 & 0.6335 & 0.8917 & 0.4624 &  \colorbox{cyan!20}{\textbf{0.5664}} & 0.8758 & 0.9577 & 0.4388 & 0.4087 & 0.8128 &  \colorbox{cyan!20}{\textbf{0.6329}} \\
\method (KL) & 0.9180 &  \colorbox{cyan!20}{\textbf{0.4992}} &  \colorbox{cyan!20}{\textbf{0.6491}} &  \colorbox{cyan!20}{\textbf{0.9060} }& 0.4524 & 0.5609 & 0.8750 &  \colorbox{cyan!20}{\textbf{0.9679}} & \colorbox{cyan!20}{\textbf{0.4603}} & 0.5199 & \colorbox{cyan!20}{\textbf{ 0.7588}} & 0.5895 \\
\midrule
 \rowcolor{beaublue!20}
\multicolumn{13}{c}{\textbf{Study on Re-weighting Mechanism Using Retain Data}} \\
% \multicolumn{13}{c}{\hdashrule[1ex]{\linewidth}{0.5pt}{1mm}} \\
\midrule
GD & 0.9080 &  \colorbox{cyan!20}{\textbf{0.4728}} &  \colorbox{cyan!20}{\textbf{0.6156}} & 0.8718 &  \colorbox{cyan!20}{\textbf{0.4439}} &  \colorbox{cyan!20}{\textbf{0.5833}} & 0.8912 & 0.9657 & \colorbox{cyan!20}{\textbf{0.4701}} & 0.4773 & 0.4238 & 0.5619 \\
\method (KL)-Retain & \colorbox{cyan!20}{\textbf{0.9180}} & 0.4643 & 0.6099 & \colorbox{cyan!20}{\textbf{0.8832}} & 0.4356 & 0.5690 &  \colorbox{cyan!20}{\textbf{0.9241}} &  \colorbox{cyan!20}{\textbf{0.9734}} &  0.4697 & \colorbox{cyan!20}{\textbf{0.4487}} &  \colorbox{cyan!20}{\textbf{0.3342}} &  \colorbox{cyan!20}{\textbf{0.5879}} \\

\bottomrule
\end{tabular}
}

\label{tab:ab_re_tofu}
\end{table}




==> LLM_Unlearning_arxiv/tables/ab_study.tex <==


\begin{table}
\caption{Ablation Study of Good Answer Type using three LLMs on TOFU dataset. FQ, MU, R-RL, F-RL represent forget quality, model utility, ROUGE-L on retain dataset and ROUGE-L on forget dataset respectively. The best performance is in \highlight[cyan!20]{\textbf{blue}}.}
% \vspace{-3mm}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|cccc|cccc|cccc}
\toprule
\textbf{Split} & \multicolumn{4}{c}{\textbf{Llama2-7B}} & \multicolumn{4}{c}{\textbf{Phi-1.5B}} & \multicolumn{4}{c}{\textbf{OPT-2.7B}} \\ 
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
\textbf{Metric} & \multicolumn{1}{c}{FQ} & \multicolumn{1}{c}{MU} & \multicolumn{1}{c}{F-RL(\(\downarrow\))} & \multicolumn{1}{c|}{R-RL} & \multicolumn{1}{c}{FQ} & \multicolumn{1}{c}{MU} & \multicolumn{1}{c}{F-RL(\(\downarrow\))} & \multicolumn{1}{c|}{R-RL} & \multicolumn{1}{c}{FQ} & \multicolumn{1}{c}{MU} & \multicolumn{1}{c}{F-RL(\(\downarrow\))} & \multicolumn{1}{c}{R-RL}   \\ 
\midrule
Original LLM & 4.4883e-06 &0.6346  & 0.9851 & 0.9833 & 0.0013 &  0.5184 & 0.9249 & 0.9293 & 0.0013 & 0.5120 & 0.7537 & 0.7494 \\  
Retained LLM & 1.0 & 0.6267 & 0.4080 & 0.9833 & 1.0 & 0.5233 & 0.4272 & 0.9269 & 1.0 & 0.5067 & 0.4217 & 0.7669  \\ 
\midrule
\method (TV)-IDK & 0.0541 & 0.6373 &\colorbox{cyan!20}{\textbf{0.4391}} & 0.8826& 0.0143 & 0.5168 & 0.4689 & 0.8155 & 0.0068 & 0.5086 & 0.5217 & 0.7067 \\

\method (KL)-IDK & 0.0286 & \colorbox{cyan!20}{\textbf{0.6393}} & 0.5199 & 0.8750 & \colorbox{cyan!20}{\textbf{0.0143}} & \colorbox{cyan!20}{\textbf{0.5180}} & \colorbox{cyan!20}{\textbf{0.4524}} & 0.7850 & 0.0286 & 0.4838 & 0.2212 & 0.4853\\
\method (JS)-IDK & 0.0541 & 0.6364 & 0.4454 & 0.8864 & 0.0068 & 0.5144  & 0.4572 & 0.8117 & \colorbox{cyan!20}{\textbf{0.0541}} &  0.4959 & 0.3104 & 0.5658 \\
\method (Pearson)-IDK & \colorbox{cyan!20}{\textbf{0.0541}} & 0.6374 & 0.4392 & 0.8857 & 0.0143& 0.5175 & 0.4591 & 0.8099 & 0.0068 & 0.5093 & \colorbox{cyan!20}{\textbf{0.5052}} & 0.7059 \\
\midrule
\method (TV)-Normal & 0.0068 & 0.6173& 0.4941& 0.9575& 0.0068 & 0.5104 & 0.4827 & 0.8245 & 0.0030 & 0.5086 & 0.5646 & 0.7355 \\ 
\method (KL)-Normal  & 0.0068 & 0.6162 &0.6273 &\colorbox{cyan!20}{\textbf{0.9719}} & 0.0068 & 0.5177 & 0.5377 & \colorbox{cyan!20}{\textbf{0.8575}} & 0.0030 & 0.5082 & 0.5642 & \colorbox{cyan!20}{\textbf{0.7474}}\\ 
\method (JS)-Normal  & 0.0143 & 0.6178 & 0.4910 & 0.9560 & 0.0013 & 0.5068 & 0.5538 & 0.7313 & 0.0013 & 0.5068 & 0.5538 & 0.7313 \\ 
\method (Pearson)-Normal   & 0.0068 & 0.6186& 0.4972& 0.9546 & 0.0030 & 0.5094 & 0.5554 & 0.7343 & 0.0030 & \colorbox{cyan!20}{\textbf{0.5094}} &0.5554 & 0.7343 \\ 

\bottomrule
\end{tabular}
}
% \vspace{-0.1in}
\label{tab:tofu-llama2-ab-answer_type}
\end{table}

==> LLM_Unlearning_arxiv/tables/baseline_comparison.tex <==
\begin{table*}[t]
\centering
% \vspace{-0.15in}
\caption{\textbf{Comparison of different loss adjustment-based baselines in terms of their requirement.} Our method relies solely on forget data and available template responses, without using the retain data or a reference model for response calibration.}
% \vspace{-2ex}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{c|cccc}
\toprule
\textbf{Baselines} & \textbf{Forget Data} & \textbf{Retain Data}  & \textbf{Reference Model}  \\ \midrule
Gradient Ascent (GA)~\cite{maini2024tofu} & \ding{51} & \ding{55}  & \ding{55} \\
Gradient Difference (GD)~\cite{maini2024tofu} & \ding{51} & \ding{51}  & \ding{55} \\
KL Minimization (KL)~\cite{maini2024tofu} & \ding{51} & \ding{51} & \ding{51} \\
Preference Optimization (PO)~\cite{maini2024tofu} & \ding{51} & \ding{51} & \ding{55}\\
Mismatch~\cite{liu2024large} & \ding{51} & \ding{51} & \ding{55}\\
Direct Preference Optimization (DPO)~\cite{rafailov2024direct} & \ding{51} & \ding{55}  & \ding{51} \\
Negative Preference Optimization (NPO)~\cite{zhang2024negative} & \ding{51} & \ding{55} & \ding{51} \\
% NPO + Fine-tune on Retain Data & \ding{51} & \ding{51}  & \ding{51} \\
Large Language Model Unlearning (LLMU)~\cite{yao2023large} & \ding{51} & \ding{51}  & \ding{51}\\
\midrule
\method (Ours) & \ding{51} & \ding{55} & \ding{55}\\

\bottomrule
\end{tabular}
}
\label{tab:baselines}
\end{table*}

==> LLM_Unlearning_arxiv/tables/divergence.tex <==
% \begin{wraptable}{r}{0.65\linewidth} 
\begin{table}[htb]
\centering
% \vspace{-0.15in}
\caption{$f_{div}$s, optimal variational $g$ ($g^*$), conjugate functions ($f^*$).}
% \vspace{-3mm}
\resizebox{0.6\linewidth}{!}{
\begin{tabular}{llll} 
 \toprule
 Name & 
 % $D_f(D^G||D^U)$  & 
 $g^*(v)$ & $\text{dom}_{f^*}$ & $f^*(u)$ \\ 
 \midrule
 Total Variation 
 % & $\int \dfrac{1}{2}|z^G-z^U|dz$ 
 &  $\dfrac{1}{2}\tanh{v}$ & $u\in [-\dfrac{1}{2}, \dfrac{1}{2}]$ & $u$\\
 Jensen-Shannon 
 % & $\dfrac{1}{2}\int z^G\log{\dfrac{2z^G}{z^G+z^U}} + z^U\log{\dfrac{2z^U}{z^G+z^U}}dz$
 & $\log{\dfrac{2}{1+e^{-v}}}$ & $u<\log{2}$  & $-\log{(2-e^{u})}$\\
 Pearson  
 % & $\int \dfrac{(z^U-z^G)^2}{z^G} dz$ 
 & $v$& $\mathbb{R}$ & $\dfrac{1}{4}u^2+u$ \\
 KL  
 % & $\int z^G \log{\dfrac{z^G}{z^U}} dz$  
 &$v$ &$\mathbb{R}$ & $e^{u-1}$\\
\bottomrule
\end{tabular}
}
\label{table:f_div}
\end{table}


==> LLM_Unlearning_arxiv/tables/unlearning_setting.tex <==
\begin{table*}[ht]
\centering
\caption{Summary of unlearning tasks, including base models, forget datasets, and evaluation metrics.}
% \vspace{-2ex}
\resizebox{\textwidth}{!}{\begin{tabular}{cccc}
\toprule
\textbf{Unlearning Task} & \textbf{Base Model} & \textbf{Forget Dataset} & \textbf{Metrics} \\ \midrule
Copyrighted Content Unlearning & OPT-2.7B, Llama2-7B & Harry Potter Series & BLEU, ROUGE\_L, PPL, Zero-shot Acc \\ 
\midrule
Entity Unlearning (TOFU) & OPT-2.7B, Llama2-7B, Phi-1.5B & TOFU-Forget01 & Forget Quality (p-value), ROUGE\_L on Forget set, Model Utility \\ 
\midrule
MUSE Benchmark & Llama2-7B & BBC News Corps & verbatim and knowledge memorization on $\mathcal{D}_f$, privacy leakage, Utility preservation \\
\bottomrule
\end{tabular}
}
\label{tab:unlearning_setting}
\end{table*}

==> src/02-related_work.tex <==
\section{Related Work}
\label{related_work}
\subsection{LLM Unlearning}
LLM unlearning approaches can be broadly categorized into three families: model-based methods, input-based methods, and data-based methods~\cite{liu2024rethinking}.

\paragraph{Model-based Methods}
Model-based approaches involve modifying the weights and/or architecture to achieve unlearning. These include gradient ascent (GA) and its variants~\cite{yao2023large,maini2024tofu,chen2023unlearn}, as well as model editing techniques~\cite{wu2023depn,ilharco2022editing,belrose2024leace}. The dominant approach among existing LLM unlearning methods is fine-tuning the original model based on a carefully designed unlearning objective function~\cite{chen2023unlearn,yao2023large,jia2024soul,li2024wmdp,yao2024machine,zhang2024negative}. A common strategy combines forgetting and retaining objectives, applying gradient ascent updates to undesirable data while using regular gradient descent on desirable data~\cite{chen2023unlearn,li2024wmdp}. The goal of GA is to maximize the loss on the forget data, essentially reversing the effect of gradient descent during training. Some methods employ custom loss functions that go beyond standard forgetting and retaining losses. For example, \cite{yao2023large} introduce a loss function with three components, where the custom loss reflects advanced techniques or regularization applied to the objectives. Other methods, such as DPO~\cite{rafailov2024direct}, KTO~\cite{ethayarajh2024kto}, and NPO~\cite{zhang2024negative}, utilize reference models to guide the unlearning process. 

\cite{chen2023unlearn} fine-tune an adapter over the unlearning objective, which acts as an unlearning layer within the LLM. Several works also employ assistant or reinforced LLMs to facilitate unlearning~\cite{ilharco2022editing,eldan2023s,huang2024offset}. For instance, \cite{ji2024reversing} introduce an assistant LLM that pursues the opposite of the unlearning goals—i.e., remembering forgotten documents and forgetting retained knowledge. The unlearned LLM is then derived by computing the logit difference between the original and assistant LLMs.

\paragraph{Data-based Methods}
Data-based methods fine-tune the LLM using a set of modified responses. This approach often begins by generating altered outputs (e.g., refusal-based responses), such as obliterated responses~\cite{choi2024snap}, inverted facts~\cite{gu2024meow}, or in-domain plausible alternatives~\cite{mekala2024alternate}. These generated responses are then used to guide the unlearning process. \cite{mekala2024alternate} propose Alternate Preference Optimization, which utilizes in-domain positive feedback on the forget set, complementing the usual negative feedback to overcome the limitations of relying solely on negative feedback during unlearning. In this work, we employ reject-based template outputs as the modified "good" responses for the forgotten samples.

\paragraph{Input-based Methods}
Input-based methods craft input instructions~\cite{pawelczyk2023context,muresanu2024unlearnable,thaker2024guardrail,bhaila2024soft,gao2024practical,liu2024large}, such as in-context examples and prompts, to steer the original LLM toward the unlearning objective without altering the model's parameters. These approaches aim to achieve unlearning in the output space rather than in the parameter space. Among these methods, a notable baseline by~\cite{liu2024large} uses an external prompt classifier as a guardrail, applying embedding corruptions to the identified prompts. The authors demonstrate that this corruption scheme results in distribution-wise similarity to the retrained model.

In this work, we propose a novel loss adjustment method for LLM unlearning, which simultaneously utilizes available example responses, effectively combining data-based and model-based methods.

\subsection{Machine Unlearning} 
In response to the data regulation requirements~\cite{hoofnagle2019european}, machine unlearning (MU) has emerged as a critical process to remove the influence of specific data points, data classes, or even higher-level data concepts from a trained machine-learning model. One direct unlearning method involves retraining the model from scratch after removing the forgotten data from the original dataset, which is often considered the gold standard~\cite{liu2024model, fan2024challenging}. However, this approach comes with significant computational demands. To alleviate this, most research focuses on developing approximate but much faster unlearning techniques, including gradient ascent~\cite{thudi2022unrolling,graves2021amnesiac}, influence unlearning~\cite{izzo2021approximate, warnecke2021machine,wu2022puma}, Fisher forgetting~\cite{becker2022evaluating,golatkar2020eternal}, finetuning-based approaches~\cite{liu2024model,fan2023salun}, and loss correction-related unlearning~\cite{adolphs2022cringe,wang2023kga, di2024label}.


